Joint Constrained Learning for Event-Event Relation Extraction

Understanding natural language involves recognizing how multiple event mentions structurally and temporally interact with each other. In this process, one can induce event complexes that organize multi-granular events with temporal order and membership relations interweaving among them. Due to the lack of jointly labeled data for these relational phenomena and the restriction on the structures they articulate, we propose a joint constrained learning framework for modeling event-event relations. Specifically, the framework enforces logical constraints within and across multiple temporal and subevent relations by converting these constraints into differentiable learning objectives. We show that our joint constrained learning approach effectively compensates for the lack of jointly labeled data, and outperforms SOTA methods on benchmarks for both temporal relation extraction and event hierarchy construction, replacing a commonly used but more expensive global inference process. We also present a promising case study showing the effectiveness of our approach in inducing event complexes on an external corpus.

==> partialLabelNoteKaifu.tex <==
\section{Future Work}
\kaifu{
\begin{enumerate}
    \item \textbf{Incorporating POS tags} We might try to concatenate POS tag embeddings with the RoBERTa embeddings to include syntactic features.
    \item \textbf{Incorporating Discourse Relations} Discourse and narrative features have been proven to be useful for event hierarchy construction. It is possible to design a framework to learn discourse relations together with event-event relation extraction.
    \item \textbf{Event Extraction} We want to design a system for event extraction without the conventional BiLSTM-CRF architecture since in event-event relation extraction we are employing a logic-driven framework that enables us to incorporate any rules we want to add. In other words, it is theoretically possible to \textbf{transfer the constraints added through CRF into logic forms} and express it in differential functions. And actually we can train a joint model for event extraction and event-event relation extraction. \textbf{Besides}, we can improve the BiLSTM by some other architecture like BERT to get contextualized representation for event extraction.
    
\end{enumerate}
\textbf{Discussion about The Partial Label in Event Extraction}
The event annotation in HiEve and MATRES is partial, i.e. many events are not considered when the annotators study event-event relations. Inspired by \cite{mayhew-etal-2019-named}, we want to develop a classifier providing confidence of a token being non-event. The confidence is designed to be incorporated in an event extraction module.

Suppose we have a model to decide if a token is an event trigger:
$$
y = \text{NN}(x)
$$
where $y=(y_1,y_2)=(\Pr(\text{trigger}|x),\Pr(\text{not trigger}|x))$
The relation between the gold label and the probabilities of the partial label $s=(s_1,s_2)$ is
$$
\begin{pmatrix}
s_1 & s_2
\end{pmatrix}
=
\begin{pmatrix}
y_1 & y_2
\end{pmatrix}
\begin{pmatrix}
1-p & p\\ 
0 & 1
\end{pmatrix}
$$
where $p=\Pr(\text{not labeled}|x\text{ is trigger})$ can be set as a trainable parameter. So we can try to add a layer 
$\begin{pmatrix}
1-p & p\\ 
0 & 1
\end{pmatrix}$ on the top of predicted probabilities and minimize the cross entropy loss of score $s$ and partial labels. When making predictions, we still use the score $y=(y_1,y_2)$.

Note that this method is valid as long as  $p<\frac12$.
}
